Anomaly Inflow Methods for SCFT Constructions in Type IIB

We extend the anomaly inflow methods developed in M-theory to SCFTs engineered via D3-branes in type IIB. We show that the 't Hooft anomalies of such SCFTs can be computed systematically from their geometric definition. Our procedure is tested in several 4d examples and applied to 2d theories obtained by wrapping D3-branes on a Riemann surface. In particular, we show how to analyze half-BPS regular punctures for 4d $\mathcal N = 4$ SYM on a Riemann surface. We discuss generalizations of this formalism to type IIB configurations with $F_3$, $H_3$ fluxes, as well as to F-theory setups.

==> sec_2d.tex <==
%!TEX root = ./IIBmain.tex

\section{Two-dimensional examples}
In this section, we apply our prescription for constructing the inflow anomaly polynomial to setups where the D3-brane stack is extended on a compact Riemann surface $\Sigma$ and a two-dimensional uncompactified worldvolume $W_2$. The six transverse directions  compose a Calabi-Yau cone, just as in the four-dimensional case. We will consider this setup with and without punctures on the Riemann surface.
\subsection{Parameterization of $\mathcal{F}_5$}
We know consider the case of a D3-brane stack wrapped on a Riemann surface with no punctures, probing a conical singularity.
Since the setup for the six transverse directions is identical to the four-dimensional worldvolume theory case, we refer the reader to the previous section for details on the Calabi-Yau cone.  To simplify the present discussion, we consider only connections associated to abelian isometries on the $SE_5$, so that all the $f_{IJ}^K$ are fixed to zero, and use the collective index $X$ for all gauge connections.

Just as before, compactification turns on background gauge connections. However, now we must distinguish field strengths on the Riemann surface from those on non-compact directions,
\begin{equation}
F^X=F_\Sigma^X +F_{2d}^X.
\end{equation}
The most general form for the field strength over the Riemann surface is $F_\Sigma^X=p^X V_\Sigma$, where $V_\Sigma$ is the volume form and $p^X$ constant coefficients. In order to construct the inflow anomaly polynomial corresponding to the two-dimensional worldvolume theory on $W_2$, the appropriate parameterization for the five-form $\mathcal{F}_5$ is to expand in powers of field strengths $F_{2d}^X$ with legs only on $W_2$:
\begin{equation}
\mathcal{F}_5=(X_5)^{2d}+F_{2d}^X (\tilde{\omega}_X)^{2d}+F_{2d}^X F_{2d}^Y (\tilde{\lambda}_{XY})^{2d}
\end{equation}
where we have defined
\begin{equation}
X_5 \equiv (V_5)^\Sigma +F_\Sigma^X (\omega_X)^\Sigma,
\end{equation}
and introduced the convention that a $"2d"$ superscript denotes gauging with connections only on $W_2$, while the $"\Sigma"$ superscript denotes gauging on the Riemann surface. With these conventions, $((...)^\Sigma)^{2d}$ would be equivalent to $(...)^g$ in the previous section. While the three-form $\omega$ is that of the previous section, we have also introduced a new three-form $\tilde \omega_X$ and a new one-form $\tilde \lambda_X$, which live in the $\Sigma \times SE_5$ space transverse to $W_2$.

%Note that by virtue of the four-dimensional closure condition $\iota_X V_5+d_5\omega_X=0$, the internal five-form $X_5$ is closed.
\subsection{Closure Constraints and Inlow Anomaly Polynomial}
We will now use the closure of 
\begin{equation}
F_5=(1+*_{10})\mathcal{F}_5
\end{equation}
to constrain the internal forms $\tilde \omega$ and $\tilde \lambda$. We will need a slightly modified expression for the ten-dimensional Hodge star, split now between the compact $\Sigma \times SE_5$ directions and the three external directions:
\begin{equation}\label{Hodge_identity_2d}
*_{10} \Big[ \alpha_{p,{\rm ext}} \, ( \beta_{q,{\rm int}})^{\rm g} \Big] 
= (-)^{q (3-p)} \, r^{7-2q} \, (*_{\rm ext}  \alpha_{p,{\rm ext}} ) \, (*_{\rm int} \, \beta_{q , {\rm int}})^{\rm g} \ 
\end{equation}
where the p-form $\alpha_{p,{\rm ext}}$ has legs on the $W_2$ and $r$ directions, and the q-form $\beta_{q,{\rm int}}$ has legs on the $SE_5$ and $\Sigma$ directions. With this identity and the closure constraints on $\omega_X$ from the four-dimensional case, we find
\begin{equation}
F_5=X_5^{2d}+F_{2d}^X \tilde{\omega}_X^{2d}+F_{2d}^X F_{2d}^Y \tilde{\lambda}_{XY}^{2d}-r^{-3}*_{ext}(1)^{2d}*_{int}X_5^{2d}-r*_{ext} F_{2d}^X *_{int} \tilde{\omega}_X^{2d}+...
\end{equation}
The Hodge dual of unity $*_{ext}(1)$ is just a volume form on the $W_2 \times [r]$ directions, call it $V_3$.
Now we can impose the closure of $F_5$. Taking the total derivative, collecting terms with the same number of external and internal legs, and setting each equal to zero, we obtain
\begin{align}
0&=r(*_{ext} F_{2d}^x)(d_7*_{int} \tilde{\omega}_x)^{2d}
\\
0&=F_{2d}^X\left[F_\Sigma^Y \iota_X \omega_Y^\Sigma -(d\omega_X)^\Sigma+d \tilde{\omega}_X \right]^{2d}-r(d_3 *_{ext} F_{2d}^X)(*_{int} \tilde{\omega}_x)^{2d}
\\
0&=r^{-3}V_3 (d_7 *_{int} X_5)^{2d}-r(*_{ext} F_{2d}^X)F_{2d}^Y (\iota_y *_{int} \tilde{\omega}_x)^{2d}
\end{align}
Tracking the number of derivatives on external directions, we set each term to zero seperately. We consider here only the constraints arising from terms containing one external derivative, as these a sufficient to compute the inflow anomaly polynomial. They are
\begin{equation}
d_{int} *_{int} \tilde{\omega}_X =0, \qquad
d\tilde{\omega}_X=(d \omega_X)^\Sigma- F_\Sigma^Y \iota_{X} \omega_{Y}^\Sigma.
\end{equation}
%the additional constraints imply that $c_x^y=0$ in $d_3 *_{ext} F_{2d}^X=c_Y^X F_{2d}^Y$, that $f^{xy}=0$ in $*_{ext} F_{2d}^X)F_{2d}^Y =V_3 f^{xy}$ and that 
%\begin{equation}
%d_7 *_{int} X_5 =V_\Sigma p^X p^Y \iota_Y *_5 \omega_X^\Sigma =0
%\end{equation}
Making use of the closure constraints on $\omega_X$ from the four-dimensional case, we find that these conditions are satisfied when $\tilde \omega_X$
%, which we can generically write as $\bar \omega_X^\Sigma+V_\Sigma \Lambda_X^\Sigma$ for some three-form $\bar \omega_X$ and one-form $\Lambda_X$ on $SE_5$, 
takes the form
\begin{equation}\label{omegatilde_solution} 
\tilde{\omega}_X=\omega_X^\Sigma+(d\Gamma_X)^\Sigma+V_\Sigma k_X,
\end{equation}
where $\Gamma_X$ has legs only on $SE_5$, and satisfies \footnote{An explicit solution for \ref{gamma_condition} an be written in terms of the killing one-forms: $\Gamma_X =-\frac{N}{16 \text{Vol}_5}p^Yk_Y k_X$. We will not need it for the present computation.}
\begin{equation}\label{gamma_condition}
d *_{SE} d \Gamma_X=p^Y \iota_X \iota_Y V_5,
\end{equation}
as well as
\begin{equation}
p^Y(\iota_X \omega_Y+\iota_Y \omega_X) +p^Y\iota_Y d \Gamma_X+dk_X=0.
\end{equation}
We can now compute the inflow anomaly polynomial.

Collecting terms in $\mathcal{F}_5 d\mathcal{F}_5$ which could have the five legs on $SE_5$ and two on $\Sigma$ required for integration on the compact directions, we obtain
\begin{align}
\int_{int} \mathcal{F}_5 d \mathcal{F}_5 = F_{2d}^X F_{2d}^Y \int_{int}  \left[ X_5 (\iota_Y \tilde{\omega}_X+ d \tilde{\lambda}_{XY})+ \tilde{\omega}_X (F_\Sigma^Z \iota_Y \omega_Z^\Sigma -(d\omega_Y)^\Sigma+d \tilde{\omega}_Y) \right]^{2d} 
\end{align}
The term containing $X_5 d \tilde{\lambda}_{XY}$ is actually a total derivative, since $dX_5=0$. So analagously to the four-dimensional case, where the inflow anomaly polynomial could be computed without specifying $\lambda_X$, here we will get a result independent of $\tilde{\lambda}_X$. To reduce further, note that we can generically write
\begin{equation}
\tilde{\omega}_X=\left[ \bar{\omega}_X + V_\Sigma \Lambda_X \right]^\Sigma,
\end{equation}
where $\bar \omega$ is the part with legs only on $SE_5$. We are left with
\begin{align}
F_{2d}^X F_{2d}^Y V_\Sigma \left[ V_5 \iota_Y \Lambda_X+p^Z \omega_Z \iota_Y \bar{\omega}_X+\bar{\omega}_X(p^Z \iota_Y \omega_Z+d\Lambda_Y +p^Z \iota_Z \bar{\omega}_Y)+k_X(d \bar{\omega}_Y-d \omega_Y) \right]^{4d}
\end{align}
From (\ref{omegatilde_solution}), we know that $\bar \omega_X=\omega_X+d \Gamma_X$, and from the four-dimensional closure condition, we have that $\iota_X V_5+d\omega_X=0$. Alongside the total symmetry of $\omega_X \iota_Y \omega_Z$ under integration, we can use these relations to write the term in brackets as
\begin{align*}
3p^Z \omega_X \iota_Y \omega_Z +2p^Z(\omega_X \iota_Z d\Gamma_Y+\omega_Z \iota_X d\Gamma_Y) +2d\Gamma_X d\Lambda_Y+p^Z d\Gamma_X \iota_Z d \Gamma_Y
\end{align*}
Two terms are total derivatives, and do not contribute. To eliminate a third, we can use the anti-symmetry of $X$ and $Z$ in $\omega_X \iota_Z d\Gamma_Y$ under integration. We are left with 
\begin{equation}
\int_{int} \mathcal{F}_5 d \mathcal{F}_5 = 3 p^X  F_{2d}^Y F_{2d}^Z \int_{V_\Sigma} V_\Sigma  \int_{V_5} \omega_X \iota_Y \omega_Z
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%It seems allowed by the AdS equations of motion to have 
%\begin{equation}
%d_3 *_{3} F_{2d}^X=c_Y^X F_{2d}^Y
%\end{equation}

%Since $(*_{ext} F_{2d}^X)F_{2d}^Y$ is a top form in the external directions, we should have
%\begin{equation}
%(*_{ext} F_{2d}^X)F_{2d}^Y =V_3 f^{xy}
%\end{equation}
%for some scalar coefficient $f^{xy}$.


 
 
 

==> topmatter.tex <==
\def\check{\textbf{CHECK!}}


%\usepackage{array,setspace,mathrsfs,amsfonts,amsmath,yfonts,dsfont,bbm,colonequals,youngtab,mathabx}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}



%\usepackage{graphicx}
%\usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{hyperref}
%\usepackage[height=8.8in,width=6.45in]{geometry}
%\def\baselinestretch{1.05}

\numberwithin{equation}{section}
\newtheorem{conj}{Conjecture}
\newtheorem{thm}{Theorem}

\def\NO#1#2{{\rm NO}(#1,#2)}
\def\CB#1{$\clubsuit$ {\bf #1} $\clubsuit$}
\def\inc#1{\vcenter{\hbox{\includegraphics[scale=.25]{#1}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ceq{\colonequals}
\def\eqc{\equalscolon}
\def\eqq{\equiv}
\def\leqs{\leqslant}
\def\geqs{\geqslant}
\def\vph{\varphi}
\def\vth{\vartheta}
\def\g{\gamma}
\def\G{\Gamma}
\def\th{\theta}
\def\Th{\Theta}
\def\tpdf{\texorpdfstring}

\DeclarePairedDelimiterX\MeijerM[3]{\lparen}{\rparen}%
{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}\delimsize\vert\,#3}

\def\zeromode#1{o\left(#1\right)}

\newcommand\MeijerG[8][]{%
  G^{\,#2,#3}_{#4,#5}\MeijerM[#1]{#6}{#7}{#8}}

\WithSuffix\newcommand\MeijerG*[7]{%
  G^{\,#1,#2}_{#3,#4}\MeijerM*{#5}{#6}{#7}}


%\def\VnoH{\VV_{\cancel{\rm H}}}
\def\VH{\VV_0}
\def\VnoH{\VV_+}
\def\VSch{\mathcal{V}_{\rm Sch}}

\newcommand{\suup}{2}
\newcommand{\sudown}{1}
\def\diag{\mathop{\mathrm{diag}}\nolimits}
\def\tr{\mathop{\mathrm{tr}}\nolimits}
\def\rank{\mathop{\mathrm{rank}}\nolimits}
\def\CP{\mathbb{CP}}
\def\GL{\mathrm{GL}}
\def\SL{\mathrm{SL}}
\def\SU{\mathrm{SU}}
\def\SO{\mathrm{SO}}
\def\USp{\mathrm{USp}}
\def\UU{\mathrm{U}}
\def\PE{\mathrm{PE}}
\def\bC{\mathbb{C}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\cH{\mathcal{H}}
\def\cDI{\mathcal{DI}}
\def\cN{\mathcal{N}}
\def\cV{\mathbb{V}}
\def\fk{\mathfrak{k}}
\def\fg{\mathfrak{g}}
\def\fh{\mathfrak{h}}
\def\sN{\text{\sffamily N}}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\vev#1{\langle#1\rangle}
\def\Hyp{\mathcal{V}}
\def\half{\frac12}
\def\S{{\mathbb S}}


\def\Vir{{\rm Vir}}
\def\AD{{\rm AD}}
\def \Rf{\mf{R}}

\def \beg#1{\begin{#1}} %This is a hack for my compiler -- doesn't have any adverse effects in general
\def \be{\beg{equation}}
\def \bea{\beg{eqnarray}}
\def \eea{\end{eqnarray}}
\def \ee{\end{equation}}

\def \a{\alpha}
\def \b{\beta}
\def \D{\Delta}

\def \PE{\mathrm{P.E.}}
%\def \NO#1{\mathop{:}\nolimits\!#1\!\mathop{:}\nolimits}
\def \goodchi{\protect\raisebox{1pt}{$\chi$}}
\def \qq{\mathbbmtt{Q}\,}
\def \Qt{\wt\QQ}
\def \St{\wt\SS}
\def \Lh{\widehat{L}}
\def \Lb{\overline{L}}
\def \af{\mf{a}}
\def \df{\mf{d}}
\def \ef{\mf{e}}
\def \gf{\mf{g}}
\def \uf{\mf{u}}
\def \glf{\mf{gl}}
\def \slf{\mf{sl}}
\def \suf{\mf{su}}
\def \sof{\mf{so}}
\def \spf{\mf{sp}}
\def \psuf{\mf{psu}}
\def \uspf{\mf{usp}}
\def \ospf{\mf{osp}}
\def \of{\mf{o}}
\def \ef{\mf{e}}
\def \hhf{\mf{h}}
\def \ceq{\colonequals}
\def \bs#1{$\clubsuit${\bf #1}$\clubsuit$}
\def \restr#1#2{{\left.\kern-\nulldelimiterspace#1\vphantom{\big|}\right|_{#2}}}

\def \Poincare{Poincar\'e}

\def \ll{\lambda}

\def \ba{{\bf a}}
\def \bb{{\bf b}}
\def \bc{{\bf c}}
\def \bd{{\bf d}}

\def \bA{{\bf A}}
\def \bB{{\bf B}}
\def \bC{{\bf C}}
\def \bD{{\bf D}}
\def \bOn{{\bf 1}}
\def \bTw{{\bf 2}}
\def \bTh{{\bf 3}}
\def \bFo{{\bf 4}}
\def \bFi{{\bf 5}}
\def \cd{{\tilde c}}

\def \hf{\frac12}
\def \qt{\frac14}

\def \mf{\mathfrak}
\def \lb{\lbrack}
\def \rb{\rbrack}
\def \nn{\nonumber}
\def \ph{\phantom}
\def \wt{\widetilde}
\def \wh{\widehat}
\def \ol{\overline}
\def \eg{{\it e.g.}}
\def \ie{{\it i.e.}}
\def \cf{{\it cf.}}
\def \Tr{{\rm Tr}}
\def \STr{{\rm STr}}
\def \til{\tilde}
\def \pr{\prime}
\def \zb{{\bar z}}
\def \db{\ol{\partial}}
\def \d{\partial}
\def \dag{\dagger}

\def \Ab{\mathbb{A}}
\def \Cb{\mathbb{C}}
\def \Eb{\mathbb{E}}
\def \Fb{\mathbb{F}}
\def \Hb{\mathbb{H}}
\def \Kb{\mathbb{K}}
\def \Mb{\mathbb{M}}
\def \Nb{\mathbb{N}}
\def \Ob{\mathbb{O}}
\def \Qb{\mathbb{Q}}
\def \Rb{\mathbb{R}}
\def \Sb{\mathbb{S}}
\def \Zb{\mathbb{Z}}


\def \AA{\mathcal{A}}
\def \BB{\mathcal{B}}
\def \CC{\mathcal{C}}
\def \DD{\mathcal{D}}
\def \EE{\mathcal{E}}
\def \FF{\mathcal{F}}
\def \GG{\mathcal{G}}
\def \HH{\mathcal{H}}
\def \II{\mathcal{I}}
\def \JJ{\mathcal{J}}
\def \KK{\mathcal{K}}
\def \LL{\mathcal{L}}
\def \MM{\mathcal{M}}
\def \NN{\mathcal{N}}
\def \OO{\mathcal{O}}
\def \PP{\mathcal{P}}
\def \QQ{\mathcal{Q}}
\def \RR{\mathcal{R}}
\def \SS{\mathcal{S}}
\def \TT{\mathcal{T}}
\def \UU{\mathcal{U}}
\def \VV{\mathcal{V}}
\def \WW{\mathcal{W}}
\def \XX{\mathcal{X}}
\def \YY{\mathcal{Y}}
\def \ZZ{\mathcal{Z}}


\def \RRR{\mathfrak{R}}

